CodeGen: An Open Large Language Model for Code with Multi-Turn Program Synthesis

Program synthesis strives to generate a computer program as a solution to a given problem specification, expressed with input-output examples or natural language descriptions. The prevalence of large language models advances the state-of-the-art for program synthesis, though limited training resources and data impede open access to such models. To democratize this, we train and release a family of large language models up to 16.1B parameters, called CODEGEN, on natural language and programming language data, and open source the training library JAXFORMER. We show the utility of the trained model by demonstrating that it is competitive with the previous state-of-the-art on zero-shot Python code generation on HumanEval. We further investigate the multi-step paradigm for program synthesis, where a single program is factorized into multiple prompts specifying subproblems. To this end, we construct an open benchmark, Multi-Turn Programming Benchmark (MTPB), consisting of 115 diverse problem sets that are factorized into multi-turn prompts. Our analysis on MTPB shows that the same intent provided to CODEGEN in multi-turn fashion significantly improves program synthesis over that provided as a single turn. We make the training library JAXFORMER and model checkpoints available as open source contribution: https://github.com/salesforce/CodeGen.

==> code/prob14.tex <==
\begin{figure*}[tb]
 \begin{minipage}[t]{0.48\textwidth}
  \centering
  \begin{lstlisting}[language=Python,linebackgroundcolor={%
    \btLstHL{36}{\color{ll2}}%
}]
# Import libraries.

import numpy as np

# Import the class LinearRegression from sklearn.

from sklearn.linear_model import LinearRegression

# Import math.

import math

# Assign integers ranging from 0 to 10 (inclusive) to "x".

x = np.arange(0, 11)

# Define a function "f" that multiplies a input argument by 2.

def f(x):
    return x * 2

# Create a numpy array of numbers "y" by applying f to each element of x.

y = f(x)

# Initialize a linear regression model.

model = LinearRegression()

# Fit the model to input x and output y (reshape both arguments with reshape(-1, 1)).

model.fit(x.reshape(-1, 1), y)

# Predict a variable "x_hat" at x=[[1]] using the fitted model.

x_hat = model.predict(x.reshape(-1, 1))

# Apply ceil() to the predicted value and print it as an integer.

print(int(math.ceil(x_hat)))
  \end{lstlisting}
  \caption*{\mpls}
 \end{minipage}
   \hspace*{.2in}
 \begin{minipage}[t]{0.48\textwidth}
  \centering
  \begin{lstlisting}[language=Python,linebackgroundcolor={%
    \btLstHL{37}{\color{ll1}}%
}]
# Import libraries.

import numpy as np

# Import the class LinearRegression from sklearn.

from sklearn.linear_model import LinearRegression

# Import math.

import math

# Assign integers ranging from 0 to 10 (inclusive) to "x".

x = np.arange(0, 11)

# Define a function "f" that multiplies a input argument by 2.

def f(x):

    return x * 2

# Create a numpy array of numbers "y" by applying f to each element of x.

y = f(x)

# Initialize a linear regression model.

model = LinearRegression()

# Fit the model to input x and output y (reshape both arguments with reshape(-1, 1)).

model.fit(x.reshape(-1, 1), y.reshape(-1, 1))

# Predict a variable "x_hat" at x=[[1]] using the fitted model.

x_hat = model.predict(np.array([[1]]))

# Apply ceil() to the predicted value and print it as an integer.

print(math.ceil(x_hat))
  \end{lstlisting}
  \caption*{\mpll}
 \end{minipage}
 \caption{Generated samples for ``Linear regression'' problem. Both models successfully load the correct model class and fit the data. However, \mpls fails to comply with the specification at prediction, where it feeds the model with the data \texttt{x}. \mpll correctly addresses the new input \texttt{x=[[1]]} for prediction.}
  \label{lst:problem_14}
\end{figure*}

==> code/prob16.tex <==
\begin{figure*}[tb]
 \begin{minipage}[t]{0.48\textwidth}
  \centering
  \begin{lstlisting}[language=Python,linebackgroundcolor={%
    \btLstHL{11-16}{\color{ll2}}%
}]
# Import libraries.

import numpy as np

# Defines a class "Person" which takes name and id as constructor arguments.

class Person:
    def __init__(self, name, id):
        self.name = name
        self.id = id

# Extend the class with a function __hash__ which uses the id property as hash value.

class Person:
    def __init__(self, name, id):
        self.name = name
        self.id = id

    def __hash__(self):
        return self.id

# |\colorbox{ll2}{Extend the class}| with a function __eq__ which returns true, if the hash value of the passed object and self are identical.

class Person:
    def __init__(self, name, id):
        self.name = name
        self.id = id

    def __eq__(self, other):
        return self.id == other.id

# Create a list "persons" with instances of Person and names "Person A", "Person B", "Person C" and ids 1, 2, 2.

persons = [Person("Person A", 1), Person("Person B", 2), Person("Person C", 2)]

# Create a set "unique_persons" of this list.

unique_persons = set(persons)

# Print the number of elements in the set.

print(len(unique_persons))
  \end{lstlisting}
  \caption*{\mpls}
 \end{minipage}
   \hspace*{.2in}
 \begin{minipage}[t]{0.48\textwidth}
  \centering
   \begin{lstlisting}[language=Python,linebackgroundcolor={%
    \btLstHL{29-30}{\color{ll1}}%
}]
# Import libraries.

import numpy as np

# Defines a class "Person" which takes name and id as constructor arguments.

class Person:
    def __init__(self, name, id):
        self.name = name
        self.id = id

# Extend the class with a function __hash__ which uses the id property as hash value.

class Person:
    def __init__(self, name, id):
        self.name = name
        self.id = id

    def __hash__(self):
        return self.id

# Extend the class with a function __eq__ which returns true, if the hash value of the passed object and self are identical.

class Person:
    def __init__(self, name, id):
        self.name = name
        self.id = id

    def __hash__(self):
        return self.id

    def __eq__(self, other):
        return self.id == other.id

# Create a list "persons" with instances of Person and names "Person A", "Person B", "Person C" and ids 1, 2, 2.

persons = [Person("Person A", 1), Person("Person B", 2), Person("Person C", 2)]

# Create a set "unique_persons" of this list.

unique_persons = set(persons)

# Print the number of elements in the set.

print(len(unique_persons))
  \end{lstlisting}
  \caption*{\mpll}
 \end{minipage}
 \caption{Generated samples for ``Dedup custom objects'' problem. Left: \mpls fails to retain the \texttt{\_\_hash\_\_} function in the third turn, which results in an error when calling the \texttt{set()} function on the list of \texttt{Person} objects. Right: \mpll keeps the function, but generates the class definition from scratch instead of extending.}
  \label{lst:problem_16}
\end{figure*}

==> code/prob39.tex <==
\begin{figure*}[tb]
 \begin{minipage}[t]{0.48\textwidth}
  \centering
  \begin{lstlisting}[language=Python,linebackgroundcolor={%
    \btLstHL{13}{\color{ll2}}%
}]
# Import libraries.

import numpy as np

# Define a string named 's' with the value 'Raising Skinny Elephants Is Utterly Boring'.

s = 'Raising Skinny Elephants Is Utterly Boring'

# Import re and compile a regular expression that matches comma and period and store the result to variable 'pattern'

import re

pattern = re.compile(r'[,.]')

# Use the variable 'pattern' to substitute all the commas and periods in the string 's' and store the result to variable 's2'

s2 = pattern.sub(' ', s)

# Split the string 's2' into a list of words with a space and store the result to variable 'words'

words = s2.split(' ')

# Print a list of integers consisting of the length of each word in 'words'

print(len(words))    
  \end{lstlisting}
  \captionsetup{labelformat=empty}
  \caption*{\mpls}
 \end{minipage}
   \hspace*{.2in}
 \begin{minipage}[t]{0.48\textwidth}
  \centering
  \begin{lstlisting}[language=Python,linebackgroundcolor={%
    \btLstHL{13}{\color{ll1}}%
}]
# Import libraries.

import numpy as np

# Define a string named 's' with the value 'Raising Skinny Elephants Is Utterly Boring'.

s = 'Raising Skinny Elephants Is Utterly Boring'

# Import re and compile a regular expression that matches comma and period and store the result to variable 'pattern'

import re

pattern = re.compile(r'[,\.]')

# Use the variable 'pattern' to substitute all the commas and periods in the string 's' and store the result to variable 's2'

s2 = pattern.sub('', s)

# Split the string 's2' into a list of words with a space and store the result to variable 'words'

words = s2.split()

# Print a list of integers consisting of the length of each word in 'words'

print(list(map(len, words)))
  \end{lstlisting}
  \caption*{\mpll}
 \end{minipage}
 \caption{Generated samples for ``Char length list'' problem. \mpls on the right makes a mistake on the regular expression to match the punctuation, while \mpll on the left correctly implements it.}
  \label{lst:problem_39}
\end{figure*}

==> code/prob4.tex <==
\begin{figure*}[h]
 \begin{minipage}[t]{0.48\textwidth}
  \centering
  \begin{lstlisting}[language=Python,linebackgroundcolor={%
    \btLstHL{17-21}{\color{ll2}}%
}]
# Import libraries.

import numpy as np

# Implement a function which returns the n-th Fibonacci number.

def fibonacci(n):
    if n == 0:
        return 0
    elif n == 1:
        return 1
    else:
        return fibonacci(n - 1) + fibonacci(n - 2)

# Implement a function that computes the square of an integer argument.

def square(n):
    if n == 0:
        return 0
    else:
        return square(n - 1) + n

# Print out the square of 10-th Fibonacci number.

print(fibonacci(10))
  \end{lstlisting}
  \caption*{\mpls}
 \end{minipage}
   \hspace*{.2in}
 \begin{minipage}[t]{0.48\textwidth}
  \centering
  \begin{lstlisting}[language=Python,linebackgroundcolor={%
    \btLstHL{17-18}{\color{ll2}}%
}]
# Import libraries.

import numpy as np

# Implement a function which returns the n-th Fibonacci number.

def fibonacci(n):
    if n == 0:
        return 0
    elif n == 1:
        return 1
    else:
        return fibonacci(n-1) + fibonacci(n-2)

# Implement a function that computes the square of an integer argument.

def square(n):
    return n * n

# Print out the square of 10-th Fibonacci number.

print(fibonacci(10) ** 2)
  \end{lstlisting}
  \caption*{\mpll}
 \end{minipage}
 \captionof{listing}{Generated samples for Squared Fibonacci problem. Left: \mpls generates a simple square function wrongly, seemingly affected by the previous fibonacci function definition. Right: \mpll correctly implements the required square function. Interestingly, however, it did not use the defined function and computed the square directly in the last turn.} 
  \label{lst:problem_4}
\end{figure*}

==> code/prob43.tex <==
\begin{figure*}[tb]
 \begin{minipage}[t]{0.48\textwidth}
  \centering
  \begin{lstlisting}[language=Python]
# Import libraries.

import numpy as np

# Create a function named 'word_weight' that takes a string as input and returns the sum of ASCII values of each alphabet in the string.

def word_weight(word):
    return sum([ord(c) for c in word])

# Given a list of strings named 'words' with the value |\colorbox{ll2}{['apple', 'banana', 'carrot']'}|, apply the function 'word_weight' to each word and store the result to variable 'weights'.

weights = []

for word in words:
    weights.append(word_weight(word))

print(weights)

# Print 'True' if the sorted 'weights' is the same as the original 'weights', otherwise 'False'.

print(sorted(weights) == weights)
  \end{lstlisting}
  \caption*{\mpls}
 \end{minipage}
   \hspace*{.2in}
 \begin{minipage}[t]{0.48\textwidth}
  \centering
  \begin{lstlisting}[language=Python,linebackgroundcolor={%
    \btLstHL{12}{\color{ll1}}%
}]
# Import libraries.

import numpy as np

# Create a function named 'word_weight' that takes a string as input and returns the sum of ASCII values of each alphabet in the string.

def word_weight(word):
    return sum(ord(c) for c in word)

# Given a list of strings named 'words' with the value ['apple', 'banana', 'carrot']', apply the function 'word_weight' to each word and store the result to variable 'weights'.

words = ['apple', 'banana', 'carrot']
weights = [word_weight(word) for word in words]
print(weights)

# Print 'True' if the sorted 'weights' is the same as the original 'weights', otherwise 'False'.

print(sorted(weights) == weights)
  \end{lstlisting}
  \caption*{\mpll}
 \end{minipage}
 \caption{Generated samples for ``Sorted word weight'' problem. \mpls on the right fails to initialize the necessary variable, while \mpll defines it in the right place.}
  \label{lst:problem_43}
\end{figure*}

==> code/prob48.tex <==
\begin{figure*}[tb]
 \begin{minipage}[t]{0.48\textwidth}
  \centering
  \begin{minted}[
frame=lines,
framesep=2mm,
baselinestretch=0.9,
fontsize=\footnotesize,
escapeinside=||,
highlightlines={11-16},
highlightcolor=ll2,
breaklines=true
]{python}
# Import libraries.

import numpy as np

# Initialize the variable named lst1 with a list ['abc', 'ab10c', 'a10bc', 'bcd'].

lst1 = ['abc', 'ab10c', 'a10bc', 'bcd']

# Create a function called num_in_str() to check whether a string contains a number.

def num_in_str(s):
    for i in s:
        if i.isdigit():
            return True
        else:
            return False

# Call the function num_in_str() to find strings in lst1 that have numbers and assign them to a list named lst2

lst2 = []
for i in lst1:
    if num_in_str(i):
        lst2.append(i)

# Print out lst2

print(lst2)

  \end{minted}
%   \caption*{\mpls}
 \end{minipage}
   \hspace*{.2in}
 \begin{minipage}[t]{0.48\textwidth}
  \centering
  \begin{minted}[
frame=lines,
framesep=2mm,
baselinestretch=0.9,
fontsize=\footnotesize,
escapeinside=||,
highlightlines={11-18},
highlightcolor=ll1,
breaklines=true
]{python}
# Import libraries.

import numpy as np

# Initialize the variable named lst1 with a list ['abc', 'ab10c', 'a10bc', 'bcd'].

lst1 = ['abc', 'ab10c', 'a10bc', 'bcd']

# Create a function called num_in_str() to check whether a string contains a number.

def num_in_str(string):
    """
    This function checks whether a string contains a number.
    """
    if any(char.isdigit() for char in string):
        return True
    else:
        return False

# Call the function num_in_str() to find strings in lst1 that have numbers and assign them to a list named lst2

lst2 = [string for string in lst1 if num_in_str(string)]

# Print out lst2

print(lst2)

  \end{minted}
%   \caption*{\mpll}
 \end{minipage}
 \captionof{listing}{Comparison of \mpls (left) and \mpll (right) via a representative example.}
  \label{lst:problem_48}
\end{figure*}

==> code/prob5.tex <==
\begin{figure*}[tb]
 \begin{minipage}[t]{0.48\textwidth}
  \centering
  \begin{lstlisting}[language=Python,linebackgroundcolor={%
    \btLstHL{11-15}{\color{ll2}}%
}]
# Import libraries.

import numpy as np

# Assign the list of numbers "[-1,-2,-3,-4]" to a variable named "my_numbers".

my_numbers = [-1,-2,-3,-4]

# Count the number of negative numbers in the list as "n_neg".

n_neg = my_numbers.count(-1)

# Count the number of positive numbers in the list as "n_pos". 

n_pos = my_numbers.count(1)

# Print out the larger number of those two.

print(f"The larger number of the two numbers is: {max(n_neg,n_pos)}")
  \end{lstlisting}
  \caption*{\mpls}
 \end{minipage}
   \hspace*{.2in}
 \begin{minipage}[t]{0.48\textwidth}
  \centering
  \begin{lstlisting}[language=Python,linebackgroundcolor={%
    \btLstHL{11-14}{\color{ll2}}%
    \btLstHL{18-21}{\color{ll2}}%
}]
# Import libraries.

import numpy as np

# Assign the list of numbers "[-1,-2,-3,-4]" to a variable named "my_numbers".

my_numbers = [-1,-2,-3,-4]

# Count the number of negative numbers in the list as "n_neg".

n_neg = 0
for i in my_numbers:
    if i < 0:
        n_neg += 1

# Count the number of positive numbers in the list as "n_pos".

n_pos = 0
for i in my_numbers:
    if i > 0:
        n_pos += 1

# Print out the larger number of those two.

if n_neg > n_pos:
    print(n_neg)
else:
    print(n_pos)
  \end{lstlisting}
  \caption*{\mpll}
 \end{minipage}
 \captionof{listing}{Generated samples for ``Compare count'' problem. While the prompt asks to count positive and negative numbers, \mpls counts the number of $1$ and $-1$. \mpll implements both specifications correctly.}
  \label{lst:problem_5}
\end{figure*}
